Development of a data infrastructure for a global data and analysis center in astroparticle physics

Nowadays astroparticle physics faces a rapid data volume increase. Meanwhile, there are still challenges of testing the theoretical models for clarifying the origin of cosmic rays by applying a multi-messenger approach, machine learning and investigation of the phenomena related to the rare statistics in detecting incoming particles. The problems are related to the accurate data mapping and data management as well as to the distributed storage and high-performance data processing. In particular, one could be interested in employing such solutions in study of air-showers induced by ultra-high energy cosmic and gamma rays, testing new hypotheses of hadronic interaction or cross-calibration of different experiments. KASCADE (Karlsruhe, Germany) and TAIGA (Tunka valley, Russia) are experiments in the field of astroparticle physics, aiming at the detection of cosmic-ray air-showers, induced by the primaries in the energy range of about hundreds TeVs to hundreds PeVs. They are located at the same latitude and have an overlap in operation runs. These factors determine the interest in performing a joint analysis of these data. In the German-Russian Astroparticle Data Life Cycle Initiative (GRADLCI), modern technologies of the distributed data management are being employed for establishing a reliable open access to the experimental cosmic-ray physics data collected by KASCADE and the Tunka-133 setup of TAIGA.

==> appl_server.tex <==
%aaplication server

\section{Application server: functionality and possible solutions}

\begin{figure}[htbp]\centering
  \includegraphics[width=1\textwidth]{img/arch_appds.png}
  \caption{
    Scheme of the data life cycle architecture for the joint analysis of KASCADE and Tunka-133 data.
    Here \textbf{S\textit{i}} stand for local data storages, \textbf{In\textit{i}} represent data sources of different types, \textbf{MDD} is a metadata description, \textbf{E\textit{i}} are metadata extractors, \textbf{A\textit{i}} are adapters that provide API for the data access, \textbf{TPL} is a template library, and \textbf{MD DB} is the metadata database.
  }
  \label{appds}
\end{figure}

Data Life Cycle (DLC) is the sequence of stages that a particular unit of data goes through from its initial generation to its archival and/or deletion.
A scheme of the data life cycle architecture for the joint analysis of KASCADE and Tunka-133 data is presented in fig.~\ref{appds}.
Its principal components are storage servers, the aggregation server, and the application server.

The aim of the aggregation server is to promote fast reliable access for the accumulated data.
The possible solutions employed for the server development could be CVMFS, PostgreSQL or TimeScale, and TPL.
The server is expected to support data caching and fast search within the metadata database.
The aggregation server is described in details in~[link,link].

The application server is expected to have the following functionality (see the grant).
Its aim is to provide user the opportunity to analyze the selected data remotely.
The server is expected to use the following computing resources: opportunistic resources on the local network, clusters (GRIDKa, BW-HPC, etc.), or external clouds (Exoscale, OpenNebula, Amazon, Google, etc.).
The load balancing is expected to be done with either HTCondor or HTCondor-based workload management systems like VCondor, Panda, or Dirac.

Features:
data mapping plugins---see Doris,
Vispa-like interface.
Add descriptions based on Wikipedia.

\section{Conclusion and outlook}

Solutions for careful sharing and managing large data volumes are in
a high demand in the field.
The Astroparticle Data Life Cycle data ecosystem is in development
by participants of GRADLC Consortium.
It is based on already existing data portal KCDC and a well-known
instruments widely used in particle physics.
The development includes building data aggregation and application
servers and a proof-of-principle joint analysis of data from KASCADE
and TAIGA experiments.
The project resources are partially provided in open access for
science and education at the astroparticle.online web-portal.
Most of the data of KASCADE are available on KCDC web-portal:
https://kcdc.ikp.kit.edu/

